Internal magnetic fields in 13 red giants detected by asteroseismology

While surface fields have been measured for stars across the HR diagram, internal magnetic fields remain largely unknown. The recent seismic detection of magnetic fields in the cores of several Kepler red giants has opened a new avenue to understand better the origin of magnetic fields and their impact on stellar structure and evolution. We aim to use asteroseismology to systematically search for internal magnetic fields in red giant stars and to determine the strengths and geometries of these fields. Magnetic fields are known to break the symmetry of rotational multiplets. In red giants, oscillation modes are mixed, behaving as pressure modes in the envelope and as gravity modes in the core. Magnetism-induced asymmetries are expected to be stronger for g-dominated modes than for p-dominated modes and to decrease with frequency. After collecting a sample of 2500 Kepler red giant stars with clear mixed-mode patterns, we specifically searched for targets among 1200 stars with dipole triplets. We identified 13 stars exhibiting clear asymmetric multiplets and measured their parameters, especially the asymmetry parameter and the magnetic frequency shift. By combining these estimates with best-fitting stellar models, we measured average core magnetic fields ranging from 20 to 150kG, corresponding to 5% to 30% of the critical field strengths. We showed that the detected core fields have various horizontal geometries, some of which significantly differ from a dipolar configuration. We found that the field strengths decrease with stellar evolution, despite the fact that the cores of these stars are contracting. Even though these stars have strong internal magnetic fields, they display normal core rotation rates, suggesting no significantly different histories of angular momentum transport compared to other red giant stars. We also discuss the possible origin of the detected fields.

==> intro.tex <==
Magnetic field and rotation are the two uncertain mechanisms of modern stellar physics \citep{Maeder2009book, McKee2007ARA&A, Ferrario2020, Kaspi2017}. 
%Magnetic fields are believed to affect the lives of stars at all evolutionary stages from star-forming molecular clouds to white dwarfs and magnetars \citep{McKee2007ARA&A, Ferrario2020, Kaspi2017}. In particular, they are expected to play a crucial role in the transport of angular momentum and chemical elements in stellar interiors \citep{Gough1998Natur}. Modelling these transport processes is key to improving the predictions of stellar evolution theory, such as the ages of stars, and will thus be helpful for exoplanet characterisation and galactic sciences.
Surface magnetic fields have been observed across the Hertzsprung-Russell diagram \citep{Landstreet1992, Donati2009}. These measurements, together with numerical simulations, establish the presence of dynamo-generated magnetic fields in convective regions \citep{Donati2009}. 
%However, the knowledge of the internal magnetic field is insufficient, and few observations have been achieved in spite of the importance. %We nevertheless rely on models to determine the intensity and topology of the internal fields, for example in the convective cores of stars with mass larger than roughly 1.4 solar masses. 
%The existence of magnetic fields in the non-convective radiative layers remain unclear in particular because the surface detections have been limited to a fraction of intermediate- and high-mass stars \citep{Braithwaite2017}. 
%Following the fossil field hypothesis, these fields originate from the stellar formation process and subsist in stellar cores to produce the observed magnetic white dwarfs and neutron stars \citep{Ferrario2020}. 
%Indirect evidences come from the internal rotation of stars measured with asteroseismology at various evolutionary stages (and in particular for the Sun). It shows that angular momentum is efficiently extracted from stellar cores and magnetic fields in radiative layers are invoked to account for the required angular momentum transport \citep{Gough1998,Fuller2019}. 
%In radiative (non-convective) zones, surface detection is limited to a fraction of intermediate- and high-mass stars and the origin of these fields remains unclear\citep{Braithwaite2017}.
A small fraction ($5-10 \%$) of intermediate- and high-mass stars with radiative envelopes harbours strong kilogauss surface fields that remain stable over decades \citep{Wade2012,Braithwaite2017}. 
These fields which are thought to result from the star formation process can subsist thanks to negligible ohmic diffusion and are potential progenitors for the magnetic white dwarfs and neutron stars \citep{Ferrario2020}. 
Numerical simulations of initial random fields relaxing into stable mixed poloidal-toroidal configurations tend to back this scenario \citep{Braithwaite2004, Becerra2022}.
%In addition, 
Another potentially widespread class of magnetic intermediate-mass stars has been identified with the detection of $\sim \!\!1$ Gauss fields in a few stars \citep{Lignieres09, Blazere2016}.


\fr{Although it seems plausible that magnetic fields pervade much of stellar interior plasmas, the lack of direct measurements of internal fields has been a significant hurdle to study their properties and their effects on stellar evolution}. 
%While the general view is that magnetic fields should pervade much of stellar interiors, the detection of the internal fields is difficult due to the opacity of the stellar envelope. The lack of direct measurements of internal fields is a significant hurdle to understanding their effects on stellar evolution. 
In a recent study, \cite{LiGang_2022_nature} reported the detection of internal magnetic fields in three stars, using magnetism-modified oscillation signals to measure the field strengths in the vicinity of hydrogen-burning shells and constrain the field topology. This breakthrough in internal magnetic field detection paves the way for magneto-asteroseismology.

%In this study, we searched for magnetism-modified oscillation signals following the phenomenon reported by \cite{LiGang_2022_nature}, and detected internal magnetic fields in \starnumber red giant stars using asteroseismology. 
%Asteroseismology is based on the idea that the oscillation waves within stars are affected by their local physical properties, providing us with a means of probing the interior environment \citep[e.g.][]{Aerts2010}. 
The Kepler mission has discovered tens of thousands of solar-like oscillators \citep{Borucki2010Sci, Bedding2010ApJ, Yu2018}, whose oscillations are excited stochastically by the outer envelope convection similar to the Sun. %Their radial ($l=0$ where $l$ is the angular degree) and quadrupole ($l=2$) pressure modes show equally spacing in frequency, which is called the large separation $\Delta\nu$ and is proportional to the square root of the mean density \citep{Huber2011ApJ}. %The power spectra show clear regular-spaced radial ($l=0$) and quadrupole ($l=2$) modes, where $l$ represents the angular degree. The large separation $\Delta \nu$ is a direct measurement of the mean density of a star hence provides accurate constraint on stellar masses and radii 
Most of these solar-like oscillators are post-main-sequence stars that exhibit mixed dipole ($l=1$) modes, which arise from the coupling between the outer pressure modes and the interior gravity modes \citep{Bedding2014}. 
%The equally-spaced frequencies predicted by asymptotic relation no longer holds\citep{shibahashi79, Tassoul1980ApJS}, but they show more complex pattern \citep[e.g.][]{Goupil13, mosser12a, mosser15}. 
Mixed modes enable us to probe the physics from the stellar core to surface, for example, to distinguish evolutionary stages or infer previous processes such as mergers or mass transfers \citep{Bedding2011, Deheuvels2022A&A, Rui2021MNRAS}. One of the significant accomplishments is the measurement of core-to-surface differential rotations \citep{Beck2012Natur, deheuvels12, Deheuvels2014, Triana2017, Gehan2018}. %It is found that main-sequence stars rotate nearly rigidly \citep{Schou1998, Gough2015, Benomar2015, Nielsen2015, LiGang2020}. After main sequence, stars tend to rotate differentially in a transition stage \citep{Deheuvels2014, Deheuvels2020}, then the core rotation rates of red giants have no correlation with their evolution and mass, despite that the cores are contracting \citep{Mosser2012,Wu2016ApJ, Gehan2018}. 


Despite advances in our observations of stellar rotation, there remains a significant discrepancy between theoretical predictions and observations. Stars appear to rotate more slowly than expected at nearly every stage of their evolution, and their differential rotations are less severe than predicted \citep{Zahn1992, Eggenberger2012, Ceillier2013, Marques2013, Ouazzani2019, LiGang2020}. %Fuller2019}.
%and the classical hydrodynamic processes \citep[e.g.][]{Zahn1992, Mathis2004, Mathis2018} cannot explain the mild differential rotation supported by observations \citep[e.g.][]{Eggenberger2012, Ceillier2013, Marques2013}. 
This suggests that there must be additional, as-yet-unknown processes responsible for carrying angular momentum inside stars, beyond the classical hydrodynamic processes \citep{Cantiello2014, Fuller2014, Belkacem2015, Spada2016, Pincon2016, Eggenberger2017, Eggenberger2019I}. 
%Internal gravity waves (IGW) excited at the bottom of the convective envelope were proposed for the additional angular momentum transport \citep{Fuller2014, Pincon2016}, but still have difficulty in more evolved red giants. Mixed modes was also considered as a candidate \citep{Belkacem2015}
%Indirect evidences come from the internal rotation of stars measured with asteroseismology at various evolutionary stages (and in particular for the Sun). It shows that angular momentum is efficiently extracted from stellar cores and magnetic fields in radiative layers are invoked to account for the required angular momentum transport \citep{Gough1998,Fuller2019}. 
One possible solution to this problem is the presence of magnetic fields in radiative cores \fr{as they are efficient at transporting angular momentum \citep{Cantiello2014, Rudiger2015,Fuller2019, Gouhier2022aa}}. 
%, which are often invoked as a way to reconcile models of angular momentum transport with %the rotation rates determined by seismology in the cores of the Sun and red giant stars %\citep{Cantiello2014, Rudiger2015,Fuller2019, Gouhier2022aa}. Magnetic fields can more %efficiently transport angular momentum through magnetohydrodynamic processes, but only %indirect clues of the presence of magnetic fields in radiative zones have been found by %the seismic measurements of rotation rates in the radiative cores of the Sun and of red %giant stars \citep{Thompson2003, Gough1998, Mosser2012, Deheuvels2014, Fuller2019}.
Furthermore, around 20\% of red giants exhibit suppressed \seb{dipole} mixed modes (with the fraction correlated with stellar mass). \seb{It was suggested that this phenomenon could be caused by}
%, which is thought to be an effect of the 
central magnetic fields, although this \seb{interpretation} is still a topic of debate \citep{Fuller2015,Stello2016,Mosser2017_dipole_modes}.


%, Gomes2020, Mathis2021, Bugnet2021, Loi2021}. 

%When the magnetic field is absent, the rotational effect lifts 
\seb{Rotation is known to lift} the degeneracy of the modes with \seb{same degree $l$ but} different azimuthal order $m$\seb{, thus producing multiplets (triplets for $l=1$ modes)}.
%and causes triplets, i.e. the peaks with the same $l$ but $m=1$, $0$, or $-1$. 
When the rotation rate is not too fast (\seb{that is, when} second-order effects are negligible),
%is not significant),
the \seb{multiplets}
%splittings 
are \seb{generally} symmetric \seb{with respect to the central $m=0$ component} 
%\comment{(This sentence is in fact not really correct, since asymmetries can arise without magnetic fields because of near-degeneracy effects. I don't know if we should mention this here, but we should not make it seem like we don't take this into account) Gang's reply: I add one sentence after to discuss the near-degeneracy effect. }. 
In this case, the asymmetry, defined as
\begin{equation}
    \delta_\mathrm{asym}=\nu_{m=-1}+\nu_{m=1}-2\nu_{m=0},
\end{equation}
\seb{vanishes}. \textcolor{black}{Near-degeneracy effect can generate asymmetries in rotational splittings, but this effect is usually minor for dipole mixed modes and 
%behaves differently when compared to the magnetic effect discussed in this study.
affects only p-dominated modes \citep{Deheuvels2017}.}

\seb{Magnetic fields can modify this simple picture.} Indeed, it has been known for decades that magnetic fields impact stellar oscillations \citep{Gough1990, Hasan2005}. \seb{Their effect on mixed modes in red giants has been addressed, considering the simple case of dipolar magnetic
fields with different radial profiles, either aligned with the rotation axis (\citealt{Gomes2020}, \citealt{Mathis2021}, \citealt{Bugnet2021}) or inclined (\citealt{Loi2021}). These studies showed that magnetic fields are expected to break the symmetry of rotational multiplets, and they produced estimates of the minimal field intensities required to detect magnetic asymmetries. Recently, \cite{LiGang_2022_nature} extended these works to \fr{arbitrary magnetic field} configurations. They found that the magnetic asymmetries of multiplets can be either positive or negative (all the configurations studied before then yielded positive asymmetries), and derived an expression relating the level of asymmetry to \fr{a weighted average of the square of the radial component of the field}. Overall, magnetic asymmetries were found to share three common features:}

%However, following the recently-developed theory by \cite{LiGang_2022_nature}, the magnetic field breaks the symmetry, and the asymmetry is
%\begin{equation}
%    \delta_\mathrm{asym} = \zeta \delta_\mathrm{g}\left(\frac{\nu_\mathrm{max}}{\nu}\right)^3,\label{eq:asymmetry_vs_freq}
%\end{equation}
%where $\delta_\mathrm{g}$ is the pure g-mode asymmetry at the frequency of the max power $\nu_\mathrm{max}$, $\nu$ is the oscillation frequency, and $\zeta$ is the fraction of g-mode inertia over the whole mode inertia \citep{Goupil13} \comment{(the reference is not correct here, the expression given corresponds to the one derived by Mathis+21. The new development in the Nature paper comes from the more general expression of $\delta_\mathrm{g}$ as a function of the field properties.)}. A g-dominated mode has $\zeta$ near one while a p-dominated mode has $\zeta$ near zero. We therefore conclude three features of the magnetism-induced asymmetry:
\begin{itemize}
    \item \seb{They have the same sign (either positive or negative) for all multiplets in a given star.}
    %asymmetry is always positive or negative in one star;
    \item \seb{They}
    %The asymmetry performs 
    \seb{vary} as 
    %a function of 
    $\nu^{-3}$, \seb{and thus decrease with frequency (in absolute value).} 
    %hence it decreases with frequency;
    \item \seb{They are larger for g-dominated modes than for p-dominated modes.}
    %The asymmetry is more significant in g-dominated modes than in p-dominated modes due to the modification of the $\zeta$ function.
\end{itemize}
\seb{If the magnetic field is strong enough, it can also significantly modify the regular spacing of g-mode period, which can be used to detect them (\citealt{LiGang_2022_nature, Bugnet2022}). This feature has been used to detect strong core fields in 11 \kepler\ red giants (\citealt{Deheuvels2023}).}

\seb{These studies naturally raise the question of the prevalence of magnetic red giants, which can shed light on the origin of these fields. In this study, we systematically searched for asymmetries  in the rotational multiplets of \kepler\ red giants with detected oscillations, and selected those that satisfy the three aforementioned features.}
%Therefore, we searched for the stars satisfying these three features among the Kepler data. 
The paper is organised as follows. \comment{In Sect.~\ref{sec:method}, we present the method we used to search for multiplet asymmetries among \kepler\ red giants and we list the underlying assumptions. This leads us to identify \starnumber targets with multiplet asymmetries that exhibit all the features expected in the presence of an internal magnetic field. In Sect.~\ref{sec:measure_field_strength}, we fit asymptotic expressions of mixed modes including rotational and magnetic perturbations to the observations for these stars. We thus obtain estimates of the average field strength in the core, as well as constraints on its horizontal topology.
%We introduce the asymptotic theory without the magnetism-induced perturbation and our data reduction in Section~\ref{sec:method}. The asymptotic expression considering both the magnetic and rotational perturbations is shown in Section~\ref{sec:measure_field_strength}, and we also show how to derive the field strength and constrain the topology by applying the theory there. 
In Sect.~\ref{sec:discussion}, we discuss the implications of these results for the origin and evolution of internal magnetic fields, and their impact on angular momentum transport.
%We discuss the results of all the \starnumber stars, including the seismic parameters, core and envelope rotation rates, field strengths, as well as the illumination to field origin in Section~\ref{sec:discussion}. The conclusion is given in Section~\ref{sec:conclusion}.
Sect.~\ref{sec:conclusion} is dedicated to conclusions.}
